Session-based Complementary Fashion Recommendations

In modern fashion e-commerce platforms, where customers can browse thousands to millions of products, recommender systems are useful tools to navigate and narrow down the vast assortment. In this scenario, complementary recommendations serve the user need to find items that can be worn together. In this paper, we present a personalized, session-based complementary item recommendation algorithm, ZSF-c, tailored for the fashion usecase. We propose a sampling strategy adopted to build the training set, which is useful when existing user interaction data cannot be directly used due to poor quality or availability. Our proposed approach shows significant improvements in terms of accuracy compared to the collaborative filtering approach, serving complementary item recommendations to our customers at the time of the experiments CF-c. The results show an offline relative uplift of +8.2% in Orders Recall@5, as well as a significant +3.24% increase in the number of purchased products measured in an online A/B test carried out in a fashion e-commerce platform with 28 million active customers.

==> extra_comments.tex <==

\iffalse
\section{EXTRA Jose comments}


%%%% OLD draft of online experiments and learnings

In businesses, you might have more item and user features, and having more complicated ways to calculate the item and
user embeddings might be desired to capture specific change in preference. These more complicated network
infrastructure affect the training time and prediction latency. Then, one has to make compromises between accuracy,
speed and simplicity.
From our experience the number of items we rank is one of the parameters we mostly play with for this.
And by having a two step approach it can be simplified? Because we can have a coarce grained reco in the top
layer and a fine grained reco with a relatively small amount of candidates.
[Number of items to rank]


In Zalando, we found that is more practical and easy to rank in a personalized way a set
[Talk about tuning these personalized methods is hard and it is good to start with the most simple approach,
which is having a two step approach]


[Talk about time to train of different methods]
[We implemented negative sampling for the training to speed up the training procedure.]

This fact might suggests that if a non-personalized solution is already in production and is performing well,
personalization could be added on top of the baseline and if the baseline is good enough it can achieve comparable or
better results than the state of the art methods
%%%%%




\begin{table}
    \caption{Training Time: for 1 epoch in minutes}
    \label{table:resultat20}
    \begin{tabular}{cccl}
        \toprule
        & Fashion-Similar & YooChoose 1/4 \\
        \midrule
        STMO & 414.23 & 41.76 \\
        STMO with N.S. & 16.83 & 11.09 \\
        \midrule
        STAMP & 414.82 & 41.93\\
        STAMP with N.S. & 16.72 & 11.64\\
        NARM & 11946.2 & 1735.6 \\
        \midrule
        STAMP + position Ranker & 4.14 & 1.40 \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}
    \caption{Prediction Time for 1024 individual requests in seconds}
    \label{table:resultat20}
    \begin{tabular}{cccl}
        \toprule
        & Fashion-Similar & YooChoose 1/4 \\
        \midrule
        I2I-CF & & \\
        STMO & &   \\
        \midrule
        STAMP & & \\
        NARM & & \\
        \midrule
        STAMP + position Ranker & & \\
        \bottomrule
    \end{tabular}
\end{table}


%%% COMMENTS ON BASELINES
However, performing this kind of test might be difficult in practice, because in businesses performing online tests
is expensive and often there are many people willing
to perform different tests.

Since one of the metrics to convince companies to perform a/b tests is offline evaluation as well as effort
to implement and put in production, this kind of test usually don't have high priority.
%%%%%%END




Business rules that we apply on the similar box.
Variant-filter (ONLY)(NO:and category-filter).

Only will be shown items that satisfy that criteria and therefore people would only click items that satisfy them.













\section{Other Benchmarks/datasets}

It is weird that many research papers describes models that are better than CF but
those methods were not better than CF in our dataset.

[WHY is this?]
One possible reason could be that our dataset is different than the next click prediction datasets like recsys15.
[But:]
Explain that there are no datasets available that are similar to our dataset. (CHECK THIS)





STAMP method for instance wanted to solve a similar problem
and they used recsys15.
Introduce recsys15, (stamp more or less tackle the same problem using recsys15)



Let's create recsys15-dedup which don't recommend itself.

\subsection{Evaluation on those datasets}

Evaluation on recsys15 and recsys15-dedup


Recommender systems have risen to major business drivers in music or video
streaming and e-commerce platforms in which too much supply has become a
structural problem. Customers are overwhelmed by massive choice when using
traditional navigational tools like attribute filters or a hierarchical category tree.
Personalization helps in identifying and serving the most relevant items for
every single customer rather than surfacing general top items. Therefore, the
whole assortment can be leveraged because long tail items can be recommended
specifically to those customers who are interested in the niche such an item
belongs to.

Recommendations can be placed in many contexts. In this study,
we are interested to recommend users items relevant given
Many approaches [stamp, narm, gru4rec] used the current user session
to


Our contributions are: \begin{itemize}
                           \item Improving state of the art recommender system by using hybrid decoder.
                           \item Studying the performance of state of the art models on out dataset.
                           \item Comparing next click prediction problem against the Recommendation problem.
\end{itemize}



Our main contributions are:
\begin{itemize}
    \item studying the performance of state of the art models on business environments
    \item Layer of item to item for improving the accuracy of state of the art recommender systems
\end{itemize}


Recent studies have been released for addressing the next click prediction problem.
Nevertheless, the next click problem can be far from the problem of recommending items in an environment like an e-commerce or songs/movies streaming sites.

We have found a significantly amount of items which appear consecutively multiple times in datasets used for comparing different recommendation algorithms. This results in the creation of sequences used for training and evaluation where the target action is exactly the same as the last action from the user.

This behaviour could be beneficial in environments like a home web page, where you might want to recall users the last action they performed on their last session. However, in some cases items appearing multiple times in a consecutive manner is the consequence of users performing double clicks in an item and the tracking recording each and every click the user performed. In that sense, learning that the user will click again might not be interesting.

On the other hand, in environments where you want to recommend relevant products to an anchor item, in for example a product page, it is not reasonable to recommend the item the user is currently seeing.

We examined YooChoose and Diginetica. We have found that the number of sequences we use for test with this pathology is for YooChoose 14\% and for Diginetica 20\%.





\begin{table}
    \caption{Personalized Similar Recommender Variants}
    \label{table:variants}
    \begin{tabular}{cccccl}
        \toprule
        &\multicolumn{2}{c}{YooChoose-Original} &\multicolumn{2}{c}{YooChoose-deduplicated}\\
        & R@20 & MRR@20 & R@20 & MRR@20\\
        \midrule
        CF I2I & 0.526 & & 0.611 & \\
        STMO & & & & \\
        STAMP & 0.7? & & 0.649 & \\
        NARM & & & & \\
        \midrule
        &\multicolumn{2}{c}{Diginetica-Original} &\multicolumn{2}{c}{Diginetica-deduplicated}\\
        & R@20 & MRR@20 & R@20 & MRR@20\\
        \midrule
        CF I2I & & & & \\
        STMO & & & & \\
        STAMP & & & & \\
        NARM & & & & \\
        \bottomrule
    \end{tabular}
\end{table}









Jerrys comments about the introduction:


In many platforms, people interact a lot with the recommendation. There are many contexts where recommendation
boxes are displayed.

% the last item the users seen in the session

% Suggested to replace the following two paragraphs: A recent study has shwon that the user session can also be
% summarized by simpler average or attention operations \cite{Liu:2018:SSA:3219819.3219950} while emphasizing more on
% the last item the users seen in the session.
% This treatment is a better match for recommenders in the fashion industry because in most of the contexts a base item
% is presented to the user prior to any recommendations.
On the other hand, a very simple approach was develop that encodes the user session only with attention and also
giving special treatment to the last item of the session \cite{Liu:2018:SSA:3219819.3219950}.

This Study is relevant for Zalando because they are considering the last item of the session as the context which is
exactly the same because the last item the user saw was the item described in the product page.

% The current strategy we describe our motivation is too specific, it sounds like:
% The GRU approaches doesn't work for our data -> we developed a method to fix that -> that's it.
% Altough it's true, it may not be able to give the readers a feeling that this work is useful to them.
% Because they don't have to deal with the zalando dataset, plus the zalando dataset is private.

% I think what can make the study sounds more useful to other people could be:
% We realized that for different datasets the performance of these session based algorithms varies,
% sometimes it's even worse than the static non-personalized methods [cite some papers].
% But it's fine, we propose a framework that improves the existing algorithms by using deep neural networks to
% generate candidates and then rank on top of it.
% We also show by experiments that the re-ranking process is non-trivial, with the proposed ranking embedding it
% achieves the best results over all datasets.
% If your dataset is more like ours, you can use i2i CF to generate candidates and still we got significant improvments.
However when evaluating those methods by offline experiments in Zalando, it was found the contrary. That means that
those methods were not performing better than collaborative filtering.

% IS MISSING THE YOUTUBE PAPER
% But I think I can mention it in the related work

Because of this, it was developed a method that works on top of the recommendation results generated by
collaborative filtering or other baselines based on session based recommendation that learns
not only the user preference but also takes into account the ranking of the candidates as a prior.
This method improves significantly over the baseline which is proven by offline experiments in
Zalando and public available datasets.







% \input{introduction}

% \input{problem_setting}

% \input{related_work}

% \input{our_approach}

% \input{system_architecture}

% \input{experiments}

% \input{conclusion_future_work}

%\input{acknowledgement}

% \input{appendix}




\fi

